Sensor Planning for Large Numbers of Robots

*The following abbreviates the abstract. Please refer to the thesis for the full abstract.* After a disaster, locating and extracting victims quickly is critical because mortality rises rapidly after the first two days. To assist search and rescue teams and improve response times, teams of camera-equipped aerial robots can engage in tasks such as mapping buildings and locating victims. These sensing tasks encapsulate difficult (NP-Hard) problems. One way to simplify planning for these tasks is to focus on maximizing sensing performance over a short time horizon. Specifically, consider the problem of how to select motions for a team of robots to maximize a notion of sensing quality (the sensing objective) over the near future, say by maximizing the amount of unknown space in a map that robots will observe over the next several seconds. By repeating this process regularly, the team can react quickly to new observations as they work to complete the sensing task. In technical terms, this planning and control process forms an example of receding-horizon control. Fortunately, common sensing objectives benefit from well-known monotonicity properties (e.g. submodularity), and greedy algorithms can exploit these monotonicity properties to solve the receding-horizon optimization problems that we study near-optimally. However, greedy algorithms typically force robots to make decisions sequentially so that planning time grows with the number of robots. Further, recent works that investigate sequential greedy planning, have demonstrated that reducing the number of sequential steps while retaining suboptimality guarantees can be hard or impossible. We demonstrate that halting growth in planning time is sometimes possible. To do so, we introduce novel greedy algorithms involving fixed numbers of sequential steps.

==> fig/communication/acceptance_rates.tex <==
% This file was created by matplotlib2tikz v0.7.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
height=\figureheight,
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={lightgray!92.0261437908!black},
xlabel={Num. Planning Rounds (\(\displaystyle n_\mathrm{d}\))},
xmin=1.51, xmax=3.49,
xtick style={color=black},
xtick={2,3},
y grid style={lightgray!92.0261437908!black},
ylabel={Acceptance Rates (by robot)},
ymin=0, ymax=0.5,
ytick style={color=black}
]
\addplot [only marks, draw=black, fill=black, colormap/viridis, mark=diamond, mark size=0.5em]
table{%
x                      y
2 0.25
3 0.333333333333333
};
\addlegendentry{$\frac{1}{2}\left(1-\frac{1}{n_\mathrm{d}}\right)$}
\draw[fill=color0,draw opacity=0] (axis cs:1.6,0) rectangle (axis cs:2.4,0.250656640289827);

\draw[fill=color0,draw opacity=0] (axis cs:2.6,0) rectangle (axis cs:3.4,0.333480687999333);
\node at (axis cs:2,0.200656640289827)[
  scale=1.0,
  anchor=north,
  text=black,
  rotate=0.0
]{\textbf{0.25}};
\node at (axis cs:3,0.283480687999333)[
  scale=1.0,
  anchor=north,
  text=black,
  rotate=0.0
]{\textbf{0.33}};
\end{axis}

\end{tikzpicture}


==> fig/communication/completion_times.tex <==
% This file was created by matplotlib2tikz v0.7.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
height=\figureheight,
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={lightgray!92.0261437908!black},
xlabel={Completion time (s)},
xmajorgrids,
xmin=728.030827665862, xmax=1394.88239544297,
xtick style={color=black},
y grid style={lightgray!92.0261437908!black},
ylabel={Num. planning rounds (\(\displaystyle n_\mathrm{d}\))},
ymin=0.5, ymax=3.5,
ytick style={color=black}
]
\addplot [black]
table {%
909.616997542573 0.85
909.616997542573 1.15
1121.62371271029 1.15
1121.62371271029 0.85
909.616997542573 0.85
};
\addplot [black]
table {%
909.616997542573 1
828.634031320505 1
};
\addplot [black]
table {%
1121.62371271029 1
1364.57096054401 1
};
\addplot [black]
table {%
828.634031320505 0.925
828.634031320505 1.075
};
\addplot [black]
table {%
1364.57096054401 0.925
1364.57096054401 1.075
};
\addplot [black, mark=*, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
inf 1
inf 1
};
\addplot [black]
table {%
824.224798584987 1.85
824.224798584987 2.15
1060.93558680856 2.15
1060.93558680856 1.85
824.224798584987 1.85
};
\addplot [black]
table {%
824.224798584987 2
758.342262564822 2
};
\addplot [black]
table {%
1060.93558680856 2
1260.24724172385 2
};
\addplot [black]
table {%
758.342262564822 1.925
758.342262564822 2.075
};
\addplot [black]
table {%
1260.24724172385 1.925
1260.24724172385 2.075
};
\addplot [black]
table {%
813.261565097056 2.85
813.261565097056 3.15
996.450806020601 3.15
996.450806020601 2.85
813.261565097056 2.85
};
\addplot [black]
table {%
813.261565097056 3
765.596695256991 3
};
\addplot [black]
table {%
996.450806020601 3
1252.46631938208 3
};
\addplot [black]
table {%
765.596695256991 2.925
765.596695256991 3.075
};
\addplot [black]
table {%
1252.46631938208 2.925
1252.46631938208 3.075
};
\addplot [black, mark=*, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
1344.45402568287 3
};
\addplot [color0]
table {%
1057.93232866904 0.85
1057.93232866904 1.15
};
\addplot [color0]
table {%
901.514099201118 1.85
901.514099201118 2.15
};
\addplot [color0]
table {%
885.914733275222 2.85
885.914733275222 3.15
};
\end{axis}

\end{tikzpicture}


==> fig/communication/messaging/messages.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}

\begin{axis}[
height=\figureheight,
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={white!69.0196078431373!black},
xlabel={Num. Agents},
xmin=8.91250938133745, xmax=112.201845430196,
xmode=log,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Messages sent},
ymin=5.08058511847032, ymax=1476205.57140071,
ymode=log,
xmajorgrids,
ymajorgrids,
ytick style={color=black}
]
\path [draw=green, fill=green, opacity=0.2, line width=0pt]
(axis cs:10,900)
--(axis cs:20,7689.40752733874)
--(axis cs:30,26568.3733177084)
--(axis cs:40,62294.873037736)
--(axis cs:50,120047.024583009)
--(axis cs:60,201398.171415843)
--(axis cs:70,313705.267673761)
--(axis cs:80,454270.865526766)
--(axis cs:90,623640.128512672)
--(axis cs:100,833332.006429047)
--(axis cs:100,820096.153570953)
--(axis cs:90,615250.591487328)
--(axis cs:80,448678.414473234)
--(axis cs:70,310103.372326239)
--(axis cs:60,198371.108584157)
--(axis cs:50,118499.855416991)
--(axis cs:40,61451.766962264)
--(axis cs:30,26333.3866822916)
--(axis cs:20,7636.67247266126)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
(axis cs:10,900)
--(axis cs:20,5651.5739198448)
--(axis cs:30,12279.5274901677)
--(axis cs:40,20217.9507360909)
--(axis cs:50,29435.9402688315)
--(axis cs:60,39742.2109873113)
--(axis cs:70,50132.2840330899)
--(axis cs:80,62292.8643423921)
--(axis cs:90,74387.1006770453)
--(axis cs:100,88055.5998555174)
--(axis cs:100,86066.8001444826)
--(axis cs:90,73185.2993229547)
--(axis cs:80,61170.3356576079)
--(axis cs:70,49209.7159669101)
--(axis cs:60,39116.9890126887)
--(axis cs:50,29044.8597311685)
--(axis cs:40,19956.8492639091)
--(axis cs:30,12193.2725098323)
--(axis cs:20,5636.8260801552)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 0pt]
(axis cs:10,630)
--(axis cs:20,2645.50477344176)
--(axis cs:30,5705.58052896138)
--(axis cs:40,9455.19805417142)
--(axis cs:50,13756.3940884743)
--(axis cs:60,18605.7395759553)
--(axis cs:70,23828.4904004114)
--(axis cs:80,29342.3163255989)
--(axis cs:90,34305.7832994343)
--(axis cs:100,40854.4165366325)
--(axis cs:100,40031.9834633675)
--(axis cs:90,33628.9367005657)
--(axis cs:80,28837.2036744011)
--(axis cs:70,23469.1095995886)
--(axis cs:60,18336.9004240447)
--(axis cs:50,13577.7659115257)
--(axis cs:40,9340.08194582858)
--(axis cs:30,5657.93947103862)
--(axis cs:20,2639.21522655824)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0pt, dash pattern=on 1pt off 1pt]
(axis cs:10,270)
--(axis cs:20,1131.9502872231)
--(axis cs:30,2450.03656252029)
--(axis cs:40,3978.88213975074)
--(axis cs:50,5873.67041591195)
--(axis cs:60,7952.80804801694)
--(axis cs:70,10025.3702495546)
--(axis cs:80,12559.2584568292)
--(axis cs:90,14884.8769034061)
--(axis cs:100,17343.2471710621)
--(axis cs:100,17023.7928289379)
--(axis cs:90,14610.8830965939)
--(axis cs:80,12345.5415431708)
--(axis cs:70,9874.7097504454)
--(axis cs:60,7850.23195198306)
--(axis cs:50,5797.04958408804)
--(axis cs:40,3935.35786024926)
--(axis cs:30,2428.92343747971)
--(axis cs:20,1129.5697127769)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt]
(axis cs:10,434.669966592386)
--(axis cs:20,2215.63042696788)
--(axis cs:30,5491.97639049365)
--(axis cs:40,10083.8246324453)
--(axis cs:50,14733.8176872128)
--(axis cs:60,20707.1187730838)
--(axis cs:70,26809.3168136134)
--(axis cs:80,33054.7432158898)
--(axis cs:90,40886.0919728146)
--(axis cs:100,48562.5022501535)
--(axis cs:100,46988.4577498465)
--(axis cs:90,39676.3080271854)
--(axis cs:80,32197.3367841102)
--(axis cs:70,25982.3631863866)
--(axis cs:60,20020.1612269162)
--(axis cs:50,14240.2623127872)
--(axis cs:40,9725.21536755475)
--(axis cs:30,5281.22360950635)
--(axis cs:20,2119.80957303212)
--(axis cs:10,407.730033407614)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
(axis cs:10,403.432109007951)
--(axis cs:20,2171.03294448317)
--(axis cs:30,5533.60404753372)
--(axis cs:40,9925.63132305812)
--(axis cs:50,15249.8877255475)
--(axis cs:60,20881.1800462425)
--(axis cs:70,27031.5865200319)
--(axis cs:80,32840.9314090504)
--(axis cs:90,41154.8861035147)
--(axis cs:100,48566.4472645341)
--(axis cs:100,46840.1127354659)
--(axis cs:90,40033.6738964853)
--(axis cs:80,31946.0285909496)
--(axis cs:70,26264.4934799681)
--(axis cs:60,20187.9399537575)
--(axis cs:50,14768.3522744525)
--(axis cs:40,9544.28867694188)
--(axis cs:30,5341.59595246628)
--(axis cs:20,2069.92705551683)
--(axis cs:10,384.967890992049)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 0pt]
(axis cs:10,415.796325780618)
--(axis cs:20,2200.83214852147)
--(axis cs:30,5288.72075722006)
--(axis cs:40,9314.78784865175)
--(axis cs:50,13391.6265269182)
--(axis cs:60,18333.7020258556)
--(axis cs:70,23720.1095748941)
--(axis cs:80,28710.5706546447)
--(axis cs:90,35021.1945368561)
--(axis cs:100,40458.0231206585)
--(axis cs:100,39724.4568793415)
--(axis cs:90,34324.1654631439)
--(axis cs:80,28229.5893453553)
--(axis cs:70,23335.9704251059)
--(axis cs:60,17986.9379741444)
--(axis cs:50,13112.6934730818)
--(axis cs:40,9096.49215134825)
--(axis cs:30,5141.75924277994)
--(axis cs:20,2109.40785147853)
--(axis cs:10,397.803674219382)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt, dash pattern=on 1pt off 1pt]
(axis cs:10,270)
--(axis cs:20,1129.11904273002)
--(axis cs:30,2436.59374119808)
--(axis cs:40,4112.91498446238)
--(axis cs:50,5943.13849656998)
--(axis cs:60,7874.1229856347)
--(axis cs:70,10080.7380439974)
--(axis cs:80,12340.8919614163)
--(axis cs:90,14919.5909035438)
--(axis cs:100,17355.7047286521)
--(axis cs:100,16986.3752713479)
--(axis cs:90,14583.6090964562)
--(axis cs:80,12113.9080385837)
--(axis cs:70,9899.74195600265)
--(axis cs:60,7762.1170143653)
--(axis cs:50,5854.78150343002)
--(axis cs:40,4062.44501553762)
--(axis cs:30,2414.76625880191)
--(axis cs:20,1124.48095726998)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt]
(axis cs:10,9)
--(axis cs:20,19.2571428571429)
--(axis cs:30,30.9761261143705)
--(axis cs:40,44.0240091978965)
--(axis cs:50,58.8722709630071)
--(axis cs:60,74.8248984967118)
--(axis cs:70,90.4538800232343)
--(axis cs:80,106.607733883376)
--(axis cs:90,123.437512164186)
--(axis cs:100,141.415346750952)
--(axis cs:100,139.144653249048)
--(axis cs:90,121.602487835814)
--(axis cs:80,105.312266116624)
--(axis cs:70,89.1061199767657)
--(axis cs:60,73.8951015032882)
--(axis cs:50,58.0477290369929)
--(axis cs:40,43.4559908021035)
--(axis cs:30,30.6238738856295)
--(axis cs:20,19.1428571428571)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
(axis cs:10,42.8447719933168)
--(axis cs:20,176.75192121621)
--(axis cs:30,381.255425640505)
--(axis cs:40,632.13919800489)
--(axis cs:50,916.364479133351)
--(axis cs:60,1242.1590934667)
--(axis cs:70,1574.2824059883)
--(axis cs:80,1951.27573908073)
--(axis cs:90,2330.48432212753)
--(axis cs:100,2720.76335359995)
--(axis cs:100,2652.83664640005)
--(axis cs:90,2280.99567787247)
--(axis cs:80,1910.20426091927)
--(axis cs:70,1550.5975940117)
--(axis cs:60,1221.8809065333)
--(axis cs:50,903.755520866649)
--(axis cs:40,624.78080199511)
--(axis cs:30,378.024574359495)
--(axis cs:20,175.60807878379)
--(axis cs:10,42.3952280066832)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 0pt]
(axis cs:10,39.4854068882424)
--(axis cs:20,165.461089757372)
--(axis cs:30,358.404150673395)
--(axis cs:40,593.02537735391)
--(axis cs:50,855.191668246173)
--(axis cs:60,1151.61054165834)
--(axis cs:70,1481.1226139413)
--(axis cs:80,1806.65806396034)
--(axis cs:90,2195.54369464558)
--(axis cs:100,2532.39945958823)
--(axis cs:100,2469.56054041177)
--(axis cs:90,2149.53630535442)
--(axis cs:80,1776.70193603966)
--(axis cs:70,1458.1973860587)
--(axis cs:60,1134.74945834166)
--(axis cs:50,843.168331753827)
--(axis cs:40,585.05462264609)
--(axis cs:30,353.915849326605)
--(axis cs:20,164.298910242628)
--(axis cs:10,38.9545931117576)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt, dash pattern=on 1pt off 1pt]
(axis cs:10,34.1866617191998)
--(axis cs:20,142.250803304171)
--(axis cs:30,307.850585421222)
--(axis cs:40,506.993362293309)
--(axis cs:50,738.58613213982)
--(axis cs:60,984.902511963989)
--(axis cs:70,1269.35459089834)
--(axis cs:80,1565.23269602324)
--(axis cs:90,1856.2458488418)
--(axis cs:100,2164.05097077406)
--(axis cs:100,2119.82902922594)
--(axis cs:90,1818.8741511582)
--(axis cs:80,1536.84730397676)
--(axis cs:70,1246.88540910166)
--(axis cs:60,968.537488036011)
--(axis cs:50,728.13386786018)
--(axis cs:40,502.326637706691)
--(axis cs:30,304.869414578778)
--(axis cs:20,140.789196695829)
--(axis cs:10,33.4533382808002)
--cycle;
\addplot [semithick, green]
table {%
10 900
20 7663.04
30 26450.88
40 61873.32
50 119273.44
60 199884.64
70 311904.32
80 451474.64
90 619445.36
100 826714.08
};
\addplot [semithick, green, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
table {%
10 900
20 5644.2
30 12236.4
40 20087.4
50 29240.4
60 39429.6
70 49671
80 61731.6
90 73786.2
100 87061.2
};
\addplot [semithick, green, dash pattern=on 2pt off 1pt on 1pt off 0pt]
table {%
10 630
20 2642.36
30 5681.76
40 9397.64
50 13667.08
60 18471.32
70 23648.8
80 29089.76
90 33967.36
100 40443.2
};
\addplot [semithick, green, dash pattern=on 1pt off 1pt]
table {%
10 270
20 1130.76
30 2439.48
40 3957.12
50 5835.36
60 7901.52
70 9950.04
80 12452.4
90 14747.88
100 17183.52
};
\addplot [semithick, red]
table {%
10 421.2
20 2167.72
30 5386.6
40 9904.52
50 14487.04
60 20363.64
70 26395.84
80 32626.04
90 40281.2
100 47775.48
};
\addplot [semithick, red, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
table {%
10 394.2
20 2120.48
30 5437.6
40 9734.96
50 15009.12
60 20534.56
70 26648.04
80 32393.48
90 40594.28
100 47703.28
};
\addplot [semithick, red, dash pattern=on 2pt off 1pt on 1pt off 0pt]
table {%
10 406.8
20 2155.12
30 5215.24
40 9205.64
50 13252.16
60 18160.32
70 23528.04
80 28470.08
90 34672.68
100 40091.24
};
\addplot [semithick, red, dash pattern=on 1pt off 1pt]
table {%
10 270
20 1126.8
30 2425.68
40 4087.68
50 5898.96
60 7818.12
70 9990.24
80 12227.4
90 14751.6
100 17171.04
};
\addplot [semithick, blue]
table {%
10 9
20 19.2
30 30.8
40 43.74
50 58.46
60 74.36
70 89.78
80 105.96
90 122.52
100 140.28
};
\addplot [semithick, blue, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
table {%
10 42.62
20 176.18
30 379.64
40 628.46
50 910.06
60 1232.02
70 1562.44
80 1930.74
90 2305.74
100 2686.8
};
\addplot [semithick, blue, dash pattern=on 2pt off 1pt on 1pt off 0pt]
table {%
10 39.22
20 164.88
30 356.16
40 589.04
50 849.18
60 1143.18
70 1469.66
80 1791.68
90 2172.54
100 2500.98
};
\addplot [semithick, blue, dash pattern=on 1pt off 1pt]
table {%
10 33.82
20 141.52
30 306.36
40 504.66
50 733.36
60 976.72
70 1258.12
80 1551.04
90 1837.56
100 2141.94
};
\end{axis}

\end{tikzpicture}


==> fig/communication/messaging/objective.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}

\begin{axis}[
height=\figureheight,
legend cell align={left},
legend columns=4,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.00,1.05)}, anchor=south west, draw=white!80!black, transpose legend},
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={white!69.0196078431373!black},
xlabel={Num. Agents},
xmin=5.5, xmax=104.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Objective (fraction of unit area)},
ymin=0.714971256238879, ymax=0.974586347275157,
xmajorgrids,
ymajorgrids,
ytick style={color=black}
]
\path [draw=green, fill=green, opacity=0.2, line width=0pt]
(axis cs:10,0.955064442497524)
--(axis cs:20,0.962785661318963)
--(axis cs:30,0.958591271642111)
--(axis cs:40,0.950941757255523)
--(axis cs:50,0.953835201064622)
--(axis cs:60,0.942033463811659)
--(axis cs:70,0.932799117623767)
--(axis cs:80,0.913059678231281)
--(axis cs:90,0.910884057472286)
--(axis cs:100,0.903167341767341)
--(axis cs:100,0.889572658232659)
--(axis cs:90,0.898503942527714)
--(axis cs:80,0.90183632176872)
--(axis cs:70,0.924112882376233)
--(axis cs:60,0.93497053618834)
--(axis cs:50,0.948240798935379)
--(axis cs:40,0.943350242744477)
--(axis cs:30,0.953316728357888)
--(axis cs:20,0.958470338681038)
--(axis cs:10,0.947527557502477)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
(axis cs:10,0.945452294581706)
--(axis cs:20,0.953956657414053)
--(axis cs:30,0.921088816511701)
--(axis cs:40,0.89681119859504)
--(axis cs:50,0.862528069837831)
--(axis cs:60,0.831900590498399)
--(axis cs:70,0.816260213670336)
--(axis cs:80,0.799009718552736)
--(axis cs:90,0.782812466913717)
--(axis cs:100,0.770886572759717)
--(axis cs:100,0.759541427240283)
--(axis cs:90,0.774111533086283)
--(axis cs:80,0.789750281447264)
--(axis cs:70,0.806899786329664)
--(axis cs:60,0.824075409501601)
--(axis cs:50,0.853723930162169)
--(axis cs:40,0.89068480140496)
--(axis cs:30,0.914107183488299)
--(axis cs:20,0.947903342585947)
--(axis cs:10,0.937691705418294)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 0pt]
(axis cs:10,0.946842243330288)
--(axis cs:20,0.897946228913635)
--(axis cs:30,0.856792818993239)
--(axis cs:40,0.831450892162482)
--(axis cs:50,0.797310269025695)
--(axis cs:60,0.781299639209468)
--(axis cs:70,0.780038813474096)
--(axis cs:80,0.760560587712159)
--(axis cs:90,0.752384407218328)
--(axis cs:100,0.752788944523225)
--(axis cs:100,0.742063055476776)
--(axis cs:90,0.743223592781672)
--(axis cs:80,0.750995412287842)
--(axis cs:70,0.771477186525904)
--(axis cs:60,0.772928360790532)
--(axis cs:50,0.788857730974305)
--(axis cs:40,0.823693107837518)
--(axis cs:30,0.84785918100676)
--(axis cs:20,0.889081771086366)
--(axis cs:10,0.939461756669712)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0pt, dash pattern=on 1pt off 1pt]
(axis cs:10,0.900323992185745)
--(axis cs:20,0.817421458168363)
--(axis cs:30,0.79263472069047)
--(axis cs:40,0.764057511465129)
--(axis cs:50,0.763783565596654)
--(axis cs:60,0.749734918128202)
--(axis cs:70,0.754339855603616)
--(axis cs:80,0.741918439437179)
--(axis cs:90,0.744564090501154)
--(axis cs:100,0.737420057804927)
--(axis cs:100,0.726771942195073)
--(axis cs:90,0.733555909498846)
--(axis cs:80,0.731537560562821)
--(axis cs:70,0.744356144396385)
--(axis cs:60,0.738357081871798)
--(axis cs:50,0.750188434403346)
--(axis cs:40,0.752142488534871)
--(axis cs:30,0.78059327930953)
--(axis cs:20,0.805354541831637)
--(axis cs:10,0.889752007814255)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt]
(axis cs:10,0.950385258383996)
--(axis cs:20,0.954457295255705)
--(axis cs:30,0.962624851444802)
--(axis cs:40,0.952586721790111)
--(axis cs:50,0.945010347897829)
--(axis cs:60,0.933350886721287)
--(axis cs:70,0.924747162032879)
--(axis cs:80,0.921814638595389)
--(axis cs:90,0.91398729632615)
--(axis cs:100,0.905082353833216)
--(axis cs:100,0.891909646166783)
--(axis cs:90,0.899888703673849)
--(axis cs:80,0.909669361404611)
--(axis cs:70,0.916296837967121)
--(axis cs:60,0.926153113278714)
--(axis cs:50,0.937049652102171)
--(axis cs:40,0.94654127820989)
--(axis cs:30,0.957195148555197)
--(axis cs:20,0.945886704744294)
--(axis cs:10,0.941450741616003)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
(axis cs:10,0.947158549810257)
--(axis cs:20,0.954859982297965)
--(axis cs:30,0.959863094374179)
--(axis cs:40,0.960434820844336)
--(axis cs:50,0.943420937887818)
--(axis cs:60,0.941544570453637)
--(axis cs:70,0.93252149577394)
--(axis cs:80,0.920907833546163)
--(axis cs:90,0.910591842770382)
--(axis cs:100,0.899883617905858)
--(axis cs:100,0.886124382094141)
--(axis cs:90,0.898640157229618)
--(axis cs:80,0.909020166453837)
--(axis cs:70,0.92386650422606)
--(axis cs:60,0.933171429546364)
--(axis cs:50,0.935623062112182)
--(axis cs:40,0.955577179155665)
--(axis cs:30,0.955072905625821)
--(axis cs:20,0.946836017702035)
--(axis cs:10,0.940229450189742)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 0pt]
(axis cs:10,0.947169664192753)
--(axis cs:20,0.955708400951721)
--(axis cs:30,0.961713981717043)
--(axis cs:40,0.954116855424827)
--(axis cs:50,0.94698291231085)
--(axis cs:60,0.940270591575637)
--(axis cs:70,0.930909959256772)
--(axis cs:80,0.923476544475749)
--(axis cs:90,0.906237348673228)
--(axis cs:100,0.905085587459794)
--(axis cs:100,0.893950412540207)
--(axis cs:90,0.893822651326772)
--(axis cs:80,0.914923455524251)
--(axis cs:70,0.920882040743228)
--(axis cs:60,0.931425408424363)
--(axis cs:50,0.939673087689151)
--(axis cs:40,0.947227144575173)
--(axis cs:30,0.955914018282957)
--(axis cs:20,0.947127599048278)
--(axis cs:10,0.939810335807247)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt, dash pattern=on 1pt off 1pt]
(axis cs:10,0.938186889348788)
--(axis cs:20,0.947369254270032)
--(axis cs:30,0.948511826463827)
--(axis cs:40,0.935380023869114)
--(axis cs:50,0.931032097629407)
--(axis cs:60,0.927844279732082)
--(axis cs:70,0.915482408471558)
--(axis cs:80,0.915199249834501)
--(axis cs:90,0.897109004150393)
--(axis cs:100,0.896019252732882)
--(axis cs:100,0.883380747267118)
--(axis cs:90,0.884702995849607)
--(axis cs:80,0.906004750165499)
--(axis cs:70,0.906225591528442)
--(axis cs:60,0.920543720267918)
--(axis cs:50,0.924071902370593)
--(axis cs:40,0.928539976130886)
--(axis cs:30,0.940116173536173)
--(axis cs:20,0.940226745729968)
--(axis cs:10,0.927105110651212)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt]
(axis cs:10,0.94103189046418)
--(axis cs:20,0.953517621998155)
--(axis cs:30,0.954249122657724)
--(axis cs:40,0.954952714996013)
--(axis cs:50,0.94573425005924)
--(axis cs:60,0.945470517940689)
--(axis cs:70,0.933154031976177)
--(axis cs:80,0.922434870699943)
--(axis cs:90,0.911027517189216)
--(axis cs:100,0.912627316033756)
--(axis cs:100,0.900156683966244)
--(axis cs:90,0.899328482810783)
--(axis cs:80,0.912945129300056)
--(axis cs:70,0.923817968023823)
--(axis cs:60,0.938909482059311)
--(axis cs:50,0.93886574994076)
--(axis cs:40,0.950499285003987)
--(axis cs:30,0.949334877342276)
--(axis cs:20,0.946954378001845)
--(axis cs:10,0.931424109535821)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
(axis cs:10,0.936786541008852)
--(axis cs:20,0.942586026087508)
--(axis cs:30,0.942602839410887)
--(axis cs:40,0.940214711254924)
--(axis cs:50,0.939377663410818)
--(axis cs:60,0.926194292516495)
--(axis cs:70,0.919464119301035)
--(axis cs:80,0.911977378122612)
--(axis cs:90,0.903237044029173)
--(axis cs:100,0.900570689618314)
--(axis cs:100,0.885757310381686)
--(axis cs:90,0.891606955970827)
--(axis cs:80,0.900658621877389)
--(axis cs:70,0.911627880698965)
--(axis cs:60,0.918513707483505)
--(axis cs:50,0.932022336589183)
--(axis cs:40,0.933097288745077)
--(axis cs:30,0.935513160589113)
--(axis cs:20,0.934809973912492)
--(axis cs:10,0.927069458991148)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 0pt]
(axis cs:10,0.914889834425338)
--(axis cs:20,0.930920161490093)
--(axis cs:30,0.938796837864068)
--(axis cs:40,0.924995030040217)
--(axis cs:50,0.929184415097051)
--(axis cs:60,0.92278717443607)
--(axis cs:70,0.915872675226162)
--(axis cs:80,0.901631954857623)
--(axis cs:90,0.889554242744052)
--(axis cs:100,0.892353507362644)
--(axis cs:100,0.881610492637356)
--(axis cs:90,0.878421757255947)
--(axis cs:80,0.892272045142377)
--(axis cs:70,0.907627324773838)
--(axis cs:60,0.91610482556393)
--(axis cs:50,0.921155584902949)
--(axis cs:40,0.918856969959783)
--(axis cs:30,0.932839162135931)
--(axis cs:20,0.922811838509907)
--(axis cs:10,0.903814165574663)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt, dash pattern=on 1pt off 1pt]
(axis cs:10,0.89108530886411)
--(axis cs:20,0.908412919070364)
--(axis cs:30,0.906676230891298)
--(axis cs:40,0.910781277380461)
--(axis cs:50,0.898371185474089)
--(axis cs:60,0.894587829641075)
--(axis cs:70,0.885352997845113)
--(axis cs:80,0.875603407152744)
--(axis cs:90,0.87654775015262)
--(axis cs:100,0.863252495700675)
--(axis cs:100,0.851735504299325)
--(axis cs:90,0.865056249847381)
--(axis cs:80,0.864916592847255)
--(axis cs:70,0.875835002154886)
--(axis cs:60,0.885976170358925)
--(axis cs:50,0.890580814525911)
--(axis cs:40,0.90303072261954)
--(axis cs:30,0.900167769108702)
--(axis cs:20,0.900207080929636)
--(axis cs:10,0.877534691135891)
--cycle;
\addplot [semithick, green]
table {%
10 0.951296
20 0.960628
30 0.955954
40 0.947146
50 0.951038
60 0.938502
70 0.928456
80 0.907448
90 0.904694
100 0.89637
};
\addlegendentry{Local-Auction}
\addplot [semithick, green, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
table {%
10 0.941572
20 0.95093
30 0.917598
40 0.893748
50 0.858126
60 0.827988
70 0.81158
80 0.79438
90 0.778462
100 0.765214
};
\addlegendentry{Local-Auction-16}
\addplot [semithick, green, dash pattern=on 2pt off 1pt on 1pt off 0pt]
table {%
10 0.943152
20 0.893514
30 0.852326
40 0.827572
50 0.793084
60 0.777114
70 0.775758
80 0.755778
90 0.747804
100 0.747426
};
\addlegendentry{Local-Auction-8}
\addplot [semithick, green, dash pattern=on 1pt off 1pt]
table {%
10 0.895038
20 0.811388
30 0.786614
40 0.7581
50 0.756986
60 0.744046
70 0.749348
80 0.736728
90 0.73906
100 0.732096
};
\addlegendentry{Local-Auction-4}
\addplot [semithick, red]
table {%
10 0.945918
20 0.950172
30 0.95991
40 0.949564
50 0.94103
60 0.929752
70 0.920522
80 0.915742
90 0.906938
100 0.898496
};
\addlegendentry{Global-Auction}
\addplot [semithick, red, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
table {%
10 0.943694
20 0.950848
30 0.957468
40 0.958006
50 0.939522
60 0.937358
70 0.928194
80 0.914964
90 0.904616
100 0.893004
};
\addlegendentry{Global-Auction-16}
\addplot [semithick, red, dash pattern=on 2pt off 1pt on 1pt off 0pt]
table {%
10 0.94349
20 0.951418
30 0.958814
40 0.950672
50 0.943328
60 0.935848
70 0.925896
80 0.9192
90 0.90003
100 0.899518
};
\addlegendentry{Global-Auction-8}
\addplot [semithick, red, dash pattern=on 1pt off 1pt]
table {%
10 0.932646
20 0.943798
30 0.944314
40 0.93196
50 0.927552
60 0.924194
70 0.910854
80 0.910602
90 0.890906
100 0.8897
};
\addlegendentry{Global-Auction-4}
\addplot [semithick, blue]
table {%
10 0.936228
20 0.950236
30 0.951792
40 0.952726
50 0.9423
60 0.94219
70 0.928486
80 0.91769
90 0.905178
100 0.906392
};
\addlegendentry{Sequential}
\addplot [semithick, blue, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
table {%
10 0.931928
20 0.938698
30 0.939058
40 0.936656
50 0.9357
60 0.922354
70 0.915546
80 0.906318
90 0.897422
100 0.893164
};
\addlegendentry{\rrsp{}-16}
\addplot [semithick, blue, dash pattern=on 2pt off 1pt on 1pt off 0pt]
table {%
10 0.909352
20 0.926866
30 0.935818
40 0.921926
50 0.92517
60 0.919446
70 0.91175
80 0.896952
90 0.883988
100 0.886982
};
\addlegendentry{\rrsp{}-8}
\addplot [semithick, blue, dash pattern=on 1pt off 1pt]
table {%
10 0.88431
20 0.90431
30 0.903422
40 0.906906
50 0.894476
60 0.890282
70 0.880594
80 0.87026
90 0.870802
100 0.857494
};
\addlegendentry{\rrsp{}-4}
\end{axis}

\end{tikzpicture}


==> fig/communication/messaging/span.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}

\begin{axis}[
height=\figureheight,
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={white!69.0196078431373!black},
xlabel={Num. Agents},
xmin=8.91250938133745, xmax=112.201845430196,
xmode=log,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Messaging span},
ymin=2.3678784177493, ymax=177.505941263161,
ymode=log,
xmajorgrids,
yminorgrids,
ytick style={color=black}
]
\path [draw=green, fill=green, opacity=0.2, line width=0pt]
(axis cs:10,10)
--(axis cs:20,20.3769309258162)
--(axis cs:30,33.0036798002977)
--(axis cs:40,46.9046222294248)
--(axis cs:50,61.5837477490934)
--(axis cs:60,77.5022068259531)
--(axis cs:70,94.2952134217424)
--(axis cs:80,108.900437181265)
--(axis cs:90,128.026934447985)
--(axis cs:100,145.878833008606)
--(axis cs:100,144.201166991394)
--(axis cs:90,126.333065552015)
--(axis cs:80,107.499562818735)
--(axis cs:70,92.8247865782576)
--(axis cs:60,76.2977931740469)
--(axis cs:50,60.7762522509066)
--(axis cs:40,46.2553777705752)
--(axis cs:30,32.5563201997023)
--(axis cs:20,20.2230690741838)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
(axis cs:10,10)
--(axis cs:20,15)
--(axis cs:30,15)
--(axis cs:40,15)
--(axis cs:50,15)
--(axis cs:60,15)
--(axis cs:70,15)
--(axis cs:80,15)
--(axis cs:90,15)
--(axis cs:100,15)
--(axis cs:100,15)
--(axis cs:90,15)
--(axis cs:80,15)
--(axis cs:70,15)
--(axis cs:60,15)
--(axis cs:50,15)
--(axis cs:40,15)
--(axis cs:30,15)
--(axis cs:20,15)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 0pt]
(axis cs:10,7)
--(axis cs:20,7)
--(axis cs:30,7)
--(axis cs:40,7)
--(axis cs:50,7)
--(axis cs:60,7)
--(axis cs:70,7)
--(axis cs:80,7)
--(axis cs:90,7)
--(axis cs:100,7)
--(axis cs:100,7)
--(axis cs:90,7)
--(axis cs:80,7)
--(axis cs:70,7)
--(axis cs:60,7)
--(axis cs:50,7)
--(axis cs:40,7)
--(axis cs:30,7)
--(axis cs:20,7)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0pt, dash pattern=on 1pt off 1pt]
(axis cs:10,3)
--(axis cs:20,3)
--(axis cs:30,3)
--(axis cs:40,3)
--(axis cs:50,3)
--(axis cs:60,3)
--(axis cs:70,3)
--(axis cs:80,3)
--(axis cs:90,3)
--(axis cs:100,3)
--(axis cs:100,3)
--(axis cs:90,3)
--(axis cs:80,3)
--(axis cs:70,3)
--(axis cs:60,3)
--(axis cs:50,3)
--(axis cs:40,3)
--(axis cs:30,3)
--(axis cs:20,3)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt]
(axis cs:10,4.82966629547096)
--(axis cs:20,5.88636196792855)
--(axis cs:30,6.74742344640559)
--(axis cs:40,7.45534536322659)
--(axis cs:50,7.56175586144379)
--(axis cs:60,7.81866605518454)
--(axis cs:70,7.80785477764673)
--(axis cs:80,8.0115749953701)
--(axis cs:90,8.3106566670345)
--(axis cs:100,8.43931778867326)
--(axis cs:100,8.20068221132674)
--(axis cs:90,8.0893433329655)
--(axis cs:80,7.78842500462991)
--(axis cs:70,7.59214522235327)
--(axis cs:60,7.58133394481546)
--(axis cs:50,7.31824413855621)
--(axis cs:40,7.18465463677341)
--(axis cs:30,6.49257655359441)
--(axis cs:20,5.63363803207145)
--(axis cs:10,4.53033370452904)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
(axis cs:10,4.48257898897724)
--(axis cs:20,5.77327890045361)
--(axis cs:30,6.83794152823172)
--(axis cs:40,7.44597375820028)
--(axis cs:50,7.76920865630638)
--(axis cs:60,8.03477115902938)
--(axis cs:70,8.088759236061)
--(axis cs:80,8.0115749953701)
--(axis cs:90,8.34902162301908)
--(axis cs:100,8.43776643944276)
--(axis cs:100,8.16223356055724)
--(axis cs:90,8.13097837698092)
--(axis cs:80,7.78842500462991)
--(axis cs:70,7.871240763939)
--(axis cs:60,7.76522884097062)
--(axis cs:50,7.55079134369362)
--(axis cs:40,7.19402624179972)
--(axis cs:30,6.60205847176828)
--(axis cs:20,5.50672109954639)
--(axis cs:10,4.27742101102276)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 0pt]
(axis cs:10,4.61995917534021)
--(axis cs:20,5.84135291760912)
--(axis cs:30,6.51075645813868)
--(axis cs:40,6.84571428571429)
--(axis cs:50,6.85714285714286)
--(axis cs:60,6.95875617133214)
--(axis cs:70,7)
--(axis cs:80,7)
--(axis cs:90,7)
--(axis cs:100,7)
--(axis cs:100,7)
--(axis cs:90,7)
--(axis cs:80,6.96)
--(axis cs:70,6.96)
--(axis cs:60,6.88124382866786)
--(axis cs:50,6.74285714285714)
--(axis cs:40,6.71428571428571)
--(axis cs:30,6.32924354186132)
--(axis cs:20,5.59864708239088)
--(axis cs:10,4.42004082465979)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt, dash pattern=on 1pt off 1pt]
(axis cs:10,3)
--(axis cs:20,3)
--(axis cs:30,3)
--(axis cs:40,3)
--(axis cs:50,3)
--(axis cs:60,3)
--(axis cs:70,3)
--(axis cs:80,3)
--(axis cs:90,3)
--(axis cs:100,3)
--(axis cs:100,3)
--(axis cs:90,3)
--(axis cs:80,3)
--(axis cs:70,3)
--(axis cs:60,3)
--(axis cs:50,3)
--(axis cs:40,3)
--(axis cs:30,3)
--(axis cs:20,3)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt]
(axis cs:10,9)
--(axis cs:20,19.2571428571429)
--(axis cs:30,30.9761261143705)
--(axis cs:40,44.0240091978965)
--(axis cs:50,58.8722709630071)
--(axis cs:60,74.8248984967118)
--(axis cs:70,90.4538800232343)
--(axis cs:80,106.607733883376)
--(axis cs:90,123.437512164186)
--(axis cs:100,141.415346750952)
--(axis cs:100,139.144653249048)
--(axis cs:90,121.602487835814)
--(axis cs:80,105.312266116624)
--(axis cs:70,89.1061199767657)
--(axis cs:60,73.8951015032882)
--(axis cs:50,58.0477290369929)
--(axis cs:40,43.4559908021035)
--(axis cs:30,30.6238738856295)
--(axis cs:20,19.1428571428571)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
(axis cs:10,14.0872955102539)
--(axis cs:20,14.7225789889772)
--(axis cs:30,14.9095695759226)
--(axis cs:40,14.8923722936566)
--(axis cs:50,14.9739266916773)
--(axis cs:60,15)
--(axis cs:70,15)
--(axis cs:80,15)
--(axis cs:90,15)
--(axis cs:100,15)
--(axis cs:100,15)
--(axis cs:90,15)
--(axis cs:80,14.96)
--(axis cs:70,15)
--(axis cs:60,14.96)
--(axis cs:50,14.9060733083227)
--(axis cs:40,14.7876277063434)
--(axis cs:30,14.8104304240774)
--(axis cs:20,14.5174210110228)
--(axis cs:10,13.6727044897461)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 0pt]
(axis cs:10,6.70985248682009)
--(axis cs:20,6.91721424112715)
--(axis cs:30,7)
--(axis cs:40,7)
--(axis cs:50,7)
--(axis cs:60,7)
--(axis cs:70,7)
--(axis cs:80,7)
--(axis cs:90,7)
--(axis cs:100,7)
--(axis cs:100,7)
--(axis cs:90,7)
--(axis cs:80,7)
--(axis cs:70,7)
--(axis cs:60,7)
--(axis cs:50,7)
--(axis cs:40,7)
--(axis cs:30,7)
--(axis cs:20,6.80278575887286)
--(axis cs:10,6.53014751317991)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt, dash pattern=on 1pt off 1pt]
(axis cs:10,2.95875617133214)
--(axis cs:20,3)
--(axis cs:30,3)
--(axis cs:40,3)
--(axis cs:50,3)
--(axis cs:60,3)
--(axis cs:70,3)
--(axis cs:80,3)
--(axis cs:90,3)
--(axis cs:100,3)
--(axis cs:100,3)
--(axis cs:90,3)
--(axis cs:80,3)
--(axis cs:70,3)
--(axis cs:60,3)
--(axis cs:50,3)
--(axis cs:40,3)
--(axis cs:30,3)
--(axis cs:20,3)
--(axis cs:10,2.88124382866786)
--cycle;
\addplot [semithick, green]
table {%
10 10
20 20.3
30 32.78
40 46.58
50 61.18
60 76.9
70 93.56
80 108.2
90 127.18
100 145.04
};
\addplot [semithick, green, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
table {%
10 10
20 15
30 15
40 15
50 15
60 15
70 15
80 15
90 15
100 15
};
\addplot [semithick, green, dash pattern=on 2pt off 1pt on 1pt off 0pt]
table {%
10 7
20 7
30 7
40 7
50 7
60 7
70 7
80 7
90 7
100 7
};
\addplot [semithick, green, dash pattern=on 1pt off 1pt]
table {%
10 3
20 3
30 3
40 3
50 3
60 3
70 3
80 3
90 3
100 3
};
\addplot [semithick, red]
table {%
10 4.68
20 5.76
30 6.62
40 7.32
50 7.44
60 7.7
70 7.7
80 7.9
90 8.2
100 8.32
};
\addplot [semithick, red, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
table {%
10 4.38
20 5.64
30 6.72
40 7.32
50 7.66
60 7.9
70 7.98
80 7.9
90 8.24
100 8.3
};
\addplot [semithick, red, dash pattern=on 2pt off 1pt on 1pt off 0pt]
table {%
10 4.52
20 5.72
30 6.42
40 6.78
50 6.8
60 6.92
70 6.98
80 6.98
90 7
100 7
};
\addplot [semithick, red, dash pattern=on 1pt off 1pt]
table {%
10 3
20 3
30 3
40 3
50 3
60 3
70 3
80 3
90 3
100 3
};
\addplot [semithick, blue]
table {%
10 9
20 19.2
30 30.8
40 43.74
50 58.46
60 74.36
70 89.78
80 105.96
90 122.52
100 140.28
};
\addplot [semithick, blue, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
table {%
10 13.88
20 14.62
30 14.86
40 14.84
50 14.94
60 14.98
70 15
80 14.98
90 15
100 15
};
\addplot [semithick, blue, dash pattern=on 2pt off 1pt on 1pt off 0pt]
table {%
10 6.62
20 6.86
30 7
40 7
50 7
60 7
70 7
80 7
90 7
100 7
};
\addplot [semithick, blue, dash pattern=on 1pt off 1pt]
table {%
10 2.92
20 3
30 3
40 3
50 3
60 3
70 3
80 3
90 3
100 3
};
\end{axis}

\end{tikzpicture}


==> fig/communication/messaging/volume.tex <==
% This file was created by tikzplotlib v0.9.4.
\begin{tikzpicture}

\begin{axis}[
height=\figureheight,
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={white!69.0196078431373!black},
xlabel={Num. Agents},
xmin=8.91250938133745, xmax=112.201845430196,
xmode=log,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Messaging volume},
ymin=16.6069871406333, ymax=81575610.0804558,
ymode=log,
xmajorgrids,
ymajorgrids,
ytick style={color=black}
]
\path [draw=green, fill=green, opacity=0.2, line width=0pt]
(axis cs:10,4545)
--(axis cs:20,78022.6733178477)
--(axis cs:30,410879.183139635)
--(axis cs:40,1273781.70557962)
--(axis cs:50,3013769.54867457)
--(axis cs:60,6025348.14219535)
--(axis cs:70,10950258.0544982)
--(axis cs:80,17806233.4630838)
--(axis cs:90,27501068.3222538)
--(axis cs:100,40495961.7549726)
--(axis cs:100,39884038.0050274)
--(axis cs:90,27139826.1177462)
--(axis cs:80,17570324.5769162)
--(axis cs:70,10824179.9455018)
--(axis cs:60,5935932.97780466)
--(axis cs:50,2973546.61132543)
--(axis cs:40,1255086.29442038)
--(axis cs:30,405375.176860365)
--(axis cs:20,77087.4466821523)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
(axis cs:10,4545)
--(axis cs:20,43013.3071301542)
--(axis cs:30,93242.6355785714)
--(axis cs:40,148281.637420823)
--(axis cs:50,210975.057326312)
--(axis cs:60,272186.222111487)
--(axis cs:70,342616.166755098)
--(axis cs:80,413249.47257063)
--(axis cs:90,497005.178082436)
--(axis cs:100,578576.754645583)
--(axis cs:100,559411.485354417)
--(axis cs:90,482409.461917564)
--(axis cs:80,401782.20742937)
--(axis cs:70,331402.033244902)
--(axis cs:60,264065.297888513)
--(axis cs:50,205381.742673688)
--(axis cs:40,144678.402579177)
--(axis cs:30,92011.8844214286)
--(axis cs:20,42745.8128698458)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 0pt]
(axis cs:10,2331)
--(axis cs:20,10181.6678658646)
--(axis cs:30,21992.7170351015)
--(axis cs:40,36323.0491388295)
--(axis cs:50,52180.9371661386)
--(axis cs:60,69456.7896171737)
--(axis cs:70,89685.8496521812)
--(axis cs:80,107091.525846436)
--(axis cs:90,126371.614973361)
--(axis cs:100,150522.923145125)
--(axis cs:100,145819.196854875)
--(axis cs:90,122852.305026639)
--(axis cs:80,104323.874153564)
--(axis cs:70,87477.0703478188)
--(axis cs:60,67792.4503828263)
--(axis cs:50,51032.2628338614)
--(axis cs:40,35643.9908611705)
--(axis cs:30,21672.6429648985)
--(axis cs:20,10122.2921341354)
--cycle;
\path [draw=green, fill=green, opacity=0.2, line width=0pt, dash pattern=on 1pt off 1pt]
(axis cs:10,513)
--(axis cs:20,2207.00535539031)
--(axis cs:30,4813.98841852699)
--(axis cs:40,7850.20972357739)
--(axis cs:50,11606.5596530177)
--(axis cs:60,15745.7813250565)
--(axis cs:70,19853.8157299466)
--(axis cs:80,24896.155583666)
--(axis cs:90,29507.4088756744)
--(axis cs:100,34433.8142169594)
--(axis cs:100,33793.2657830406)
--(axis cs:90,28958.6311243256)
--(axis cs:80,24470.164416334)
--(axis cs:70,19553.7042700534)
--(axis cs:60,15542.4586749435)
--(axis cs:50,11453.9203469823)
--(axis cs:40,7762.67027642261)
--(axis cs:30,4772.13158147301)
--(axis cs:20,2202.27464460969)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt]
(axis cs:10,3536.69966592386)
--(axis cs:20,37098.8128035059)
--(axis cs:30,139803.528958505)
--(axis cs:40,344501.403705129)
--(axis cs:50,624322.287390549)
--(axis cs:60,1052132.97871103)
--(axis cs:70,1580036.16616814)
--(axis cs:80,2217892.54605945)
--(axis cs:90,3089994.35559153)
--(axis cs:100,4068862.45938482)
--(axis cs:100,3915378.10061518)
--(axis cs:90,2984090.20440847)
--(axis cs:80,2150328.73394055)
--(axis cs:70,1523376.47383186)
--(axis cs:60,1011417.34128897)
--(axis cs:50,599832.432609451)
--(axis cs:40,330176.196294871)
--(axis cs:30,133491.111041495)
--(axis cs:20,35182.9471964941)
--(axis cs:10,3267.30033407614)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
(axis cs:10,3224.32109007951)
--(axis cs:20,36208.0731401333)
--(axis cs:30,141091.460698838)
--(axis cs:40,338508.182899222)
--(axis cs:50,649827.289591707)
--(axis cs:60,1063941.53891153)
--(axis cs:70,1599511.29497564)
--(axis cs:80,2202226.44102047)
--(axis cs:90,3113385.72424381)
--(axis cs:100,4068125.4473501)
--(axis cs:100,3899374.5126499)
--(axis cs:90,3014848.47575619)
--(axis cs:80,2132002.11897953)
--(axis cs:70,1546643.78502436)
--(axis cs:60,1022596.06108847)
--(axis cs:50,626039.750408293)
--(axis cs:40,323397.977100778)
--(axis cs:30,135338.619301162)
--(axis cs:20,34186.4068598667)
--(axis cs:10,3039.67890992049)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 0pt]
(axis cs:10,3347.96325780618)
--(axis cs:20,36802.0069271058)
--(axis cs:30,133714.724738185)
--(axis cs:40,313629.281187978)
--(axis cs:50,557112.105166281)
--(axis cs:60,910074.051723016)
--(axis cs:70,1365978.15597853)
--(axis cs:80,1872392.90540099)
--(axis cs:90,2558392.7321698)
--(axis cs:100,3257162.87355079)
--(axis cs:100,3190995.96644921)
--(axis cs:90,2501672.0278302)
--(axis cs:80,1836954.05459901)
--(axis cs:70,1341013.56402147)
--(axis cs:60,890314.068276984)
--(axis cs:50,543528.294833719)
--(axis cs:40,305037.518812022)
--(axis cs:30,129310.795261815)
--(axis cs:20,34973.5130728942)
--(axis cs:10,3168.03674219382)
--cycle;
\path [draw=red, fill=red, opacity=0.2, line width=0pt, dash pattern=on 1pt off 1pt]
(axis cs:10,1890)
--(axis cs:20,15369.2867327161)
--(axis cs:30,48160.698986387)
--(axis cs:40,105460.007108598)
--(axis cs:50,184148.678955262)
--(axis cs:60,283025.816097337)
--(axis cs:70,412881.536255677)
--(axis cs:80,562750.723170019)
--(axis cs:90,751448.490513438)
--(axis cs:100,946707.340584146)
--(axis cs:100,918263.939415854)
--(axis cs:90,727751.069486562)
--(axis cs:80,548437.556829981)
--(axis cs:70,402768.983744323)
--(axis cs:60,277521.783902663)
--(axis cs:50,180421.641044738)
--(axis cs:40,103680.952891402)
--(axis cs:30,47560.181013613)
--(axis cs:20,15280.3132672839)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt]
(axis cs:10,45)
--(axis cs:20,192.955061295197)
--(axis cs:30,466.885931551083)
--(axis cs:40,890.796985575981)
--(axis cs:50,1485.74057099192)
--(axis cs:60,2282.47901409305)
--(axis cs:70,3216.54713843371)
--(axis cs:80,4339.76973115858)
--(axis cs:90,5697.34465353175)
--(axis cs:100,7234.80532416563)
--(axis cs:100,7115.11467583437)
--(axis cs:90,5601.09534646825)
--(axis cs:80,4278.79026884142)
--(axis cs:70,3164.41286156629)
--(axis cs:60,2248.20098590695)
--(axis cs:50,1458.81942900808)
--(axis cs:40,877.043014424019)
--(axis cs:30,460.874068448917)
--(axis cs:20,191.564938704803)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
(axis cs:10,42.8447719933168)
--(axis cs:20,176.75192121621)
--(axis cs:30,381.255425640505)
--(axis cs:40,632.13919800489)
--(axis cs:50,916.364479133351)
--(axis cs:60,1242.1590934667)
--(axis cs:70,1574.2824059883)
--(axis cs:80,1951.27573908073)
--(axis cs:90,2330.48432212753)
--(axis cs:100,2720.76335359995)
--(axis cs:100,2652.83664640005)
--(axis cs:90,2280.99567787247)
--(axis cs:80,1910.20426091927)
--(axis cs:70,1550.5975940117)
--(axis cs:60,1221.8809065333)
--(axis cs:50,903.755520866649)
--(axis cs:40,624.78080199511)
--(axis cs:30,378.024574359495)
--(axis cs:20,175.60807878379)
--(axis cs:10,42.3952280066832)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt, dash pattern=on 2pt off 1pt on 1pt off 0pt]
(axis cs:10,39.4854068882424)
--(axis cs:20,165.461089757372)
--(axis cs:30,358.404150673395)
--(axis cs:40,593.02537735391)
--(axis cs:50,855.191668246173)
--(axis cs:60,1151.61054165834)
--(axis cs:70,1481.1226139413)
--(axis cs:80,1806.65806396034)
--(axis cs:90,2195.54369464558)
--(axis cs:100,2532.39945958823)
--(axis cs:100,2469.56054041177)
--(axis cs:90,2149.53630535442)
--(axis cs:80,1776.70193603966)
--(axis cs:70,1458.1973860587)
--(axis cs:60,1134.74945834166)
--(axis cs:50,843.168331753827)
--(axis cs:40,585.05462264609)
--(axis cs:30,353.915849326605)
--(axis cs:20,164.298910242628)
--(axis cs:10,38.9545931117576)
--cycle;
\path [draw=blue, fill=blue, opacity=0.2, line width=0pt, dash pattern=on 1pt off 1pt]
(axis cs:10,34.1866617191998)
--(axis cs:20,142.250803304171)
--(axis cs:30,307.850585421222)
--(axis cs:40,506.993362293309)
--(axis cs:50,738.58613213982)
--(axis cs:60,984.902511963989)
--(axis cs:70,1269.35459089834)
--(axis cs:80,1565.23269602324)
--(axis cs:90,1856.2458488418)
--(axis cs:100,2164.05097077406)
--(axis cs:100,2119.82902922594)
--(axis cs:90,1818.8741511582)
--(axis cs:80,1536.84730397676)
--(axis cs:70,1246.88540910166)
--(axis cs:60,968.537488036011)
--(axis cs:50,728.13386786018)
--(axis cs:40,502.326637706691)
--(axis cs:30,304.869414578778)
--(axis cs:20,140.789196695829)
--(axis cs:10,33.4533382808002)
--cycle;
\addplot [semithick, green]
table {%
10 4545
20 77555.06
30 408127.18
40 1264434
50 2993658.08
60 5980640.56
70 10887219
80 17688279.02
90 27320447.22
100 40189999.88
};
\addplot [semithick, green, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
table {%
10 4545
20 42879.56
30 92627.26
40 146480.02
50 208178.4
60 268125.76
70 337009.1
80 407515.84
90 489707.32
100 568994.12
};
\addplot [semithick, green, dash pattern=on 2pt off 1pt on 1pt off 0pt]
table {%
10 2331
20 10151.98
30 21832.68
40 35983.52
50 51606.6
60 68624.62
70 88581.46
80 105707.7
90 124611.96
100 148171.06
};
\addplot [semithick, green, dash pattern=on 1pt off 1pt]
table {%
10 513
20 2204.64
30 4793.06
40 7806.44
50 11530.24
60 15644.12
70 19703.76
80 24683.16
90 29233.02
100 34113.54
};
\addplot [semithick, red]
table {%
10 3402
20 36140.88
30 136647.32
40 337338.8
50 612077.36
60 1031775.16
70 1551706.32
80 2184110.64
90 3037042.28
100 3992120.28
};
\addplot [semithick, red, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
table {%
10 3132
20 35197.24
30 138215.04
40 330953.08
50 637933.52
60 1043268.8
70 1573077.54
80 2167114.28
90 3064117.1
100 3983749.98
};
\addplot [semithick, red, dash pattern=on 2pt off 1pt on 1pt off 0pt]
table {%
10 3258
20 35887.76
30 131512.76
40 309333.4
50 550320.2
60 900194.06
70 1353495.86
80 1854673.48
90 2530032.38
100 3224079.42
};
\addplot [semithick, red, dash pattern=on 1pt off 1pt]
table {%
10 1890
20 15324.8
30 47860.44
40 104570.48
50 182285.16
60 280273.8
70 407825.26
80 555594.14
90 739599.78
100 932485.64
};
\addplot [semithick, blue]
table {%
10 45
20 192.26
30 463.88
40 883.92
50 1472.28
60 2265.34
70 3190.48
80 4309.28
90 5649.22
100 7174.96
};
\addplot [semithick, blue, dash pattern=on 2pt off 1pt on 1pt off 1pt on 1pt off 0pt]
table {%
10 42.62
20 176.18
30 379.64
40 628.46
50 910.06
60 1232.02
70 1562.44
80 1930.74
90 2305.74
100 2686.8
};
\addplot [semithick, blue, dash pattern=on 2pt off 1pt on 1pt off 0pt]
table {%
10 39.22
20 164.88
30 356.16
40 589.04
50 849.18
60 1143.18
70 1469.66
80 1791.68
90 2172.54
100 2500.98
};
\addplot [semithick, blue, dash pattern=on 1pt off 1pt]
table {%
10 33.82
20 141.52
30 306.36
40 504.66
50 733.36
60 976.72
70 1258.12
80 1551.04
90 1837.56
100 2141.94
};
\end{axis}

\end{tikzpicture}


==> fig/communication/messaging_completion.tex <==
% This file was created by matplotlib2tikz v0.7.6.
\begin{tikzpicture}

\definecolor{color1}{rgb}{1,0.752941176470588,0.796078431372549}
\definecolor{color0}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.67843137254902,0.847058823529412,0.901960784313726}

\begin{axis}[
height=\figureheight,
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={lightgray!92.0261437908!black},
xmin=713.741153796415, xmax=1499.9,
xtick style={color=black},
xlabel={Completion Time (s)},
xmajorgrids,
y grid style={lightgray!92.0261437908!black},
ymin=0.35, ymax=3.65,
ytick={0.85, 1.15, 1.85, 2.15, 2.85, 3.15},
yticklabels={
  Msgs. Disabled{,} $n_\mathrm{d}\!=\!1$,
  Msgs. Enabled{,} $n_\mathrm{d}\!=\!1$,
  Msgs. Disabled{,} $n_\mathrm{d}\!=\!2$,
  Msgs. Enabled{,} $n_\mathrm{d}\!=\!2$,
  Msgs. Disabled{,} $n_\mathrm{d}\!=\!3$,
  Msgs. Enabled{,} $n_\mathrm{d}\!=\!3$
},
ytick style={color=black}
]
\addplot [thick, black]
table {%
968.421709963383 0.85
824.630703665925 0.85
};
\addplot [thick, black]
table {%
1229.45083830831 0.85
1462.41737825005 0.85
};
\addplot [thick, black]
table {%
824.630703665925 0.79375
824.630703665925 0.90625
};
\addplot [thick, black]
table {%
1462.41737825005 0.79375
1462.41737825005 0.90625
};
\addplot [thick, black, mark=*, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
inf 0.85
inf 0.85
};
\addplot [thick, black]
table {%
915.952952693343 1.15
834.664840854614 1.15
};
\addplot [thick, black]
table {%
1126.53028563257 1.15
1373.55945668531 1.15
};
\addplot [thick, black]
table {%
834.664840854614 1.09375
834.664840854614 1.20625
};
\addplot [thick, black]
table {%
1373.55945668531 1.09375
1373.55945668531 1.20625
};
\addplot [thick, black, mark=*, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
inf 1.15
inf 1.15
};
\addplot [thick, black]
table {%
891.556808453766 1.85
798.093214663733 1.85
};
\addplot [thick, black]
table {%
1145.93939879746 1.85
1315.45865956889 1.85
};
\addplot [thick, black]
table {%
798.093214663733 1.79375
798.093214663733 1.90625
};
\addplot [thick, black]
table {%
1315.45865956889 1.79375
1315.45865956889 1.90625
};
\addplot [thick, black]
table {%
828.510497611454 2.15
764.468327652525 2.15
};
\addplot [thick, black]
table {%
1067.39182760943 2.15
1269.85910806444 2.15
};
\addplot [thick, black]
table {%
764.468327652525 2.09375
764.468327652525 2.20625
};
\addplot [thick, black]
table {%
1269.85910806444 2.09375
1269.85910806444 2.20625
};
\addplot [thick, black]
table {%
861.37276355218 2.85
749.649571647519 2.85
};
\addplot [thick, black]
table {%
1077.85912378912 2.85
1325.38005786883 2.85
};
\addplot [thick, black]
table {%
749.649571647519 2.79375
749.649571647519 2.90625
};
\addplot [thick, black]
table {%
1325.38005786883 2.79375
1325.38005786883 2.90625
};
\addplot [thick, black, mark=*, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
1453.88947462625 2.85
1467.81792866961 2.85
};
\addplot [thick, black]
table {%
816.981668168851 3.15
769.178898075703 3.15
};
\addplot [thick, black]
table {%
1007.93511795016 3.15
1263.80293589593 3.15
};
\addplot [thick, black]
table {%
769.178898075703 3.09375
769.178898075703 3.20625
};
\addplot [thick, black]
table {%
1263.80293589593 3.09375
1263.80293589593 3.20625
};
\addplot [thick, black, mark=*, mark size=3, mark options={solid,fill opacity=0}, only marks]
table {%
1455.1099785072 3.15
};
\path [draw=black, fill=color1, thick]
(axis cs:968.421709963383,0.7375)
--(axis cs:968.421709963383,0.9625)
--(axis cs:1229.45083830831,0.9625)
--(axis cs:1229.45083830831,0.7375)
--(axis cs:968.421709963383,0.7375)
--cycle;
\path [draw=black, fill=color2, thick]
(axis cs:915.952952693343,1.0375)
--(axis cs:915.952952693343,1.2625)
--(axis cs:1126.53028563257,1.2625)
--(axis cs:1126.53028563257,1.0375)
--(axis cs:915.952952693343,1.0375)
--cycle;
\path [draw=black, fill=color1, thick]
(axis cs:891.556808453766,1.7375)
--(axis cs:891.556808453766,1.9625)
--(axis cs:1145.93939879746,1.9625)
--(axis cs:1145.93939879746,1.7375)
--(axis cs:891.556808453766,1.7375)
--cycle;
\path [draw=black, fill=color2, thick]
(axis cs:828.510497611454,2.0375)
--(axis cs:828.510497611454,2.2625)
--(axis cs:1067.39182760943,2.2625)
--(axis cs:1067.39182760943,2.0375)
--(axis cs:828.510497611454,2.0375)
--cycle;
\path [draw=black, fill=color1, thick]
(axis cs:861.37276355218,2.7375)
--(axis cs:861.37276355218,2.9625)
--(axis cs:1077.85912378912,2.9625)
--(axis cs:1077.85912378912,2.7375)
--(axis cs:861.37276355218,2.7375)
--cycle;
\path [draw=black, fill=color2, thick]
(axis cs:816.981668168851,3.0375)
--(axis cs:816.981668168851,3.2625)
--(axis cs:1007.93511795016,3.2625)
--(axis cs:1007.93511795016,3.0375)
--(axis cs:816.981668168851,3.0375)
--cycle;
\addplot [thick, color0]
table {%
1055.17577226721 0.7375
1055.17577226721 0.9625
};
\addplot [thick, color0]
table {%
1062.84442425493 1.0375
1062.84442425493 1.2625
};
\addplot [thick, color0]
table {%
955.417745898204 1.7375
955.417745898204 1.9625
};
\addplot [thick, color0]
table {%
907.304690391315 2.0375
907.304690391315 2.2625
};
\addplot [thick, color0]
table {%
941.174531211203 2.7375
941.174531211203 2.9625
};
\addplot [thick, color0]
table {%
889.675177631703 3.0375
889.675177631703 3.2625
};
\end{axis}

\end{tikzpicture}


==> fig/scalable_multi-agent_coverage/compare_solvers/edge_weight_frequency.tex <==
% This file was created by matplotlib2tikz v0.6.15.
\begin{tikzpicture}

\begin{axis}[
xlabel={Edge weight (redundancy)},
xlabel near ticks,
ylabel={Frequency},
ylabel near ticks,
xmin=0, xmax=0.04,
ymin=0, ymax=70000,
xticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2
},
scaled x ticks=false,
axis on top,
width=\figurewidth,
height=\figureheight,
tick pos=both
]
\draw[draw=black,fill=blue] (axis cs:0,0) rectangle (axis cs:0.00198,62427);
\draw[draw=black,fill=blue] (axis cs:0.00198,0) rectangle (axis cs:0.00396,3100);
\draw[draw=black,fill=blue] (axis cs:0.00396,0) rectangle (axis cs:0.00594,2649);
\draw[draw=black,fill=blue] (axis cs:0.00594,0) rectangle (axis cs:0.00792,2460);
\draw[draw=black,fill=blue] (axis cs:0.00792,0) rectangle (axis cs:0.0099,2297);
\draw[draw=black,fill=blue] (axis cs:0.0099,0) rectangle (axis cs:0.01188,2094);
\draw[draw=black,fill=blue] (axis cs:0.01188,0) rectangle (axis cs:0.01386,2151);
\draw[draw=black,fill=blue] (axis cs:0.01386,0) rectangle (axis cs:0.01584,2179);
\draw[draw=black,fill=blue] (axis cs:0.01584,0) rectangle (axis cs:0.01782,2205);
\draw[draw=black,fill=blue] (axis cs:0.01782,0) rectangle (axis cs:0.0198,2164);
\draw[draw=black,fill=blue] (axis cs:0.0198,0) rectangle (axis cs:0.02178,2289);
\draw[draw=black,fill=blue] (axis cs:0.02178,0) rectangle (axis cs:0.02376,2685);
\draw[draw=black,fill=blue] (axis cs:0.02376,0) rectangle (axis cs:0.02574,3077);
\draw[draw=black,fill=blue] (axis cs:0.02574,0) rectangle (axis cs:0.02772,3688);
\draw[draw=black,fill=blue] (axis cs:0.02772,0) rectangle (axis cs:0.0297,4483);
\draw[draw=black,fill=blue] (axis cs:0.0297,0) rectangle (axis cs:0.03168,5346);
\draw[draw=black,fill=blue] (axis cs:0.03168,0) rectangle (axis cs:0.03366,6140);
\draw[draw=black,fill=blue] (axis cs:0.03366,0) rectangle (axis cs:0.03564,5858);
\draw[draw=black,fill=blue] (axis cs:0.03564,0) rectangle (axis cs:0.03762,4140);
\draw[draw=black,fill=blue] (axis cs:0.03762,0) rectangle (axis cs:0.0396,1068);
\end{axis}

\end{tikzpicture}


==> fig/scalable_multi-agent_coverage/compare_solvers/results.tex <==
% This file was created by matplotlib2tikz v0.6.15.
\begin{tikzpicture}

\begin{axis}[
xlabel={Area coverage},
xlabel near ticks,
xmin=0.65, xmax=1,
ymin=0.5, ymax=6.5,
axis on top,
width=\figurewidth,
height=\figureheight,
ytick={1,2,3,4,5,6},
yticklabels={
  Random,
  Myopic,
  \textbf{\rsp[][\textbf]{} $\bm{\numrounds{=}2}$},
  \textbf{\rsp[][\textbf]{} $\bm{\numrounds{=}4}$},
  \textbf{\rsp[][\textbf]{} $\bm{\numrounds{=}8}$},
  \textcolor{red}{Sequential}
},
tick pos=both
]
\addplot [blue, forget plot]
table {%
0.75405 0.75
0.75405 1.25
0.8087 1.25
0.8087 0.75
0.75405 0.75
};
\addplot [blue, dashed, forget plot]
table {%
0.75405 1
0.6987 1
};
\addplot [blue, dashed, forget plot]
table {%
0.8087 1
0.8764 1
};
\addplot [black, forget plot]
table {%
0.6987 0.875
0.6987 1.125
};
\addplot [black, forget plot]
table {%
0.8764 0.875
0.8764 1.125
};
\addplot [red, forget plot]
table {%
0.77845 0.75
0.77845 1.25
};
\addplot [blue, forget plot]
table {%
0.737425 1.75
0.737425 2.25
0.781875 2.25
0.781875 1.75
0.737425 1.75
};
\addplot [blue, dashed, forget plot]
table {%
0.737425 2
0.6816 2
};
\addplot [blue, dashed, forget plot]
table {%
0.781875 2
0.8368 2
};
\addplot [black, forget plot]
table {%
0.6816 1.875
0.6816 2.125
};
\addplot [black, forget plot]
table {%
0.8368 1.875
0.8368 2.125
};
\addplot [red, forget plot]
table {%
0.75955 1.75
0.75955 2.25
};
\addplot [blue, forget plot]
table {%
0.85105 2.75
0.85105 3.25
0.881725 3.25
0.881725 2.75
0.85105 2.75
};
\addplot [blue, dashed, forget plot]
table {%
0.85105 3
0.8071 3
};
\addplot [blue, dashed, forget plot]
table {%
0.881725 3
0.9078 3
};
\addplot [black, forget plot]
table {%
0.8071 2.875
0.8071 3.125
};
\addplot [black, forget plot]
table {%
0.9078 2.875
0.9078 3.125
};
\addplot [red, forget plot]
table {%
0.86645 2.75
0.86645 3.25
};
\addplot [blue, mark=+, mark size=3, mark options={solid,draw=black}, only marks, forget plot]
table {%
0.7898 3
0.7819 3
};
\addplot [blue, forget plot]
table {%
0.904075 3.75
0.904075 4.25
0.929675 4.25
0.929675 3.75
0.904075 3.75
};
\addplot [blue, dashed, forget plot]
table {%
0.904075 4
0.875 4
};
\addplot [blue, dashed, forget plot]
table {%
0.929675 4
0.9539 4
};
\addplot [black, forget plot]
table {%
0.875 3.875
0.875 4.125
};
\addplot [black, forget plot]
table {%
0.9539 3.875
0.9539 4.125
};
\addplot [red, forget plot]
table {%
0.91925 3.75
0.91925 4.25
};
\addplot [blue, mark=+, mark size=3, mark options={solid,draw=black}, only marks, forget plot]
table {%
0.8599 4
0.8531 4
};
\addplot [blue, forget plot]
table {%
0.93045 4.75
0.93045 5.25
0.951225 5.25
0.951225 4.75
0.93045 4.75
};
\addplot [blue, dashed, forget plot]
table {%
0.93045 5
0.9067 5
};
\addplot [blue, dashed, forget plot]
table {%
0.951225 5
0.9727 5
};
\addplot [black, forget plot]
table {%
0.9067 4.875
0.9067 5.125
};
\addplot [black, forget plot]
table {%
0.9727 4.875
0.9727 5.125
};
\addplot [red, forget plot]
table {%
0.94075 4.75
0.94075 5.25
};
\addplot [blue, mark=+, mark size=3, mark options={solid,draw=black}, only marks, forget plot]
table {%
0.8753 5
};
\addplot [blue, forget plot]
table {%
0.953 5.75
0.953 6.25
0.970425 6.25
0.970425 5.75
0.953 5.75
};
\addplot [blue, dashed, forget plot]
table {%
0.953 6
0.9346 6
};
\addplot [blue, dashed, forget plot]
table {%
0.970425 6
0.985 6
};
\addplot [black, forget plot]
table {%
0.9346 5.875
0.9346 6.125
};
\addplot [black, forget plot]
table {%
0.985 5.875
0.985 6.125
};
\addplot [red, forget plot]
table {%
0.96115 5.75
0.96115 6.25
};
\addplot [blue, mark=+, mark size=3, mark options={solid,draw=black}, only marks, forget plot]
table {%
0.9232 6
0.9243 6
};
\end{axis}

\end{tikzpicture}


==> fig/scalable_multi-agent_coverage/compare_solvers/total_graph_weight_frequency.tex <==
% This file was created by matplotlib2tikz v0.6.15.
\begin{tikzpicture}

\begin{axis}[
xlabel={Redundancy graph weight},
xlabel near ticks,
ylabel={Frequency},
ylabel near ticks,
xmin=10, xmax=18,
ymin=0, ymax=15,
axis on top,
width=\figurewidth,
height=\figureheight,
tick pos=both
]
\draw[draw=black,fill=blue] (axis cs:10.7846,0) rectangle (axis cs:11.10065,2);
\draw[draw=black,fill=blue] (axis cs:11.10065,0) rectangle (axis cs:11.4167,4);
\draw[draw=black,fill=blue] (axis cs:11.4167,0) rectangle (axis cs:11.73275,2);
\draw[draw=black,fill=blue] (axis cs:11.73275,0) rectangle (axis cs:12.0488,2);
\draw[draw=black,fill=blue] (axis cs:12.0488,0) rectangle (axis cs:12.36485,4);
\draw[draw=black,fill=blue] (axis cs:12.36485,0) rectangle (axis cs:12.6809,3);
\draw[draw=black,fill=blue] (axis cs:12.6809,0) rectangle (axis cs:12.99695,8);
\draw[draw=black,fill=blue] (axis cs:12.99695,0) rectangle (axis cs:13.313,8);
\draw[draw=black,fill=blue] (axis cs:13.313,0) rectangle (axis cs:13.62905,7);
\draw[draw=black,fill=blue] (axis cs:13.62905,0) rectangle (axis cs:13.9451,6);
\draw[draw=black,fill=blue] (axis cs:13.9451,0) rectangle (axis cs:14.26115,10);
\draw[draw=black,fill=blue] (axis cs:14.26115,0) rectangle (axis cs:14.5772,14);
\draw[draw=black,fill=blue] (axis cs:14.5772,0) rectangle (axis cs:14.89325,6);
\draw[draw=black,fill=blue] (axis cs:14.89325,0) rectangle (axis cs:15.2093,4);
\draw[draw=black,fill=blue] (axis cs:15.2093,0) rectangle (axis cs:15.52535,5);
\draw[draw=black,fill=blue] (axis cs:15.52535,0) rectangle (axis cs:15.8414,5);
\draw[draw=black,fill=blue] (axis cs:15.8414,0) rectangle (axis cs:16.15745,3);
\draw[draw=black,fill=blue] (axis cs:16.15745,0) rectangle (axis cs:16.4735,3);
\draw[draw=black,fill=blue] (axis cs:16.4735,0) rectangle (axis cs:16.78955,3);
\draw[draw=black,fill=blue] (axis cs:16.78955,0) rectangle (axis cs:17.1056,1);
\end{axis}

\end{tikzpicture}


==> fig/target_tracking/entropy_by_solver_plot.tex <==
% This file was created by tikzplotlib v0.8.7.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
height=\figureheight,
legend cell align={left},
legend columns=4,
legend style={fill opacity=0.8, transpose legend, draw opacity=1, text opacity=1, draw=white!80.0!black},
legend image post style={scale=0.5}, % resize legend entries
tick align=inside,
tick pos=left,
width=\figurewidth,
x grid style={white!69.01960784313725!black},
xlabel={Number of robots},
xlabel near ticks,
xtick={8,16,24,32,40},
xmajorgrids,
xmin=6.4, xmax=41.6,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Entropy per target (bits)},
ylabel near ticks,
ymajorgrids,
ymin=2.25400156907432, ymax=2.87339313533498,
ytick style={color=black}
]
\addplot [semithick, black]
table {%
8 2.55621392898628
16 2.40764100601117
24 2.36123636928243
32 2.40119212558279
40 2.34046973703584
};
\addlegendentry{\textbf{\rsp[][\textbf]{} $\bm{\numrounds=2}$}}
\addplot [semithick, black, dashed]
table {%
8 2.50932106193458
16 2.37106433972607
24 2.30337156715658
32 2.34360081591599
40 2.30747222107126
};
\addlegendentry{\textbf{\rsp[][\textbf]{} $\bm{\numrounds=4}$}}
\addplot [semithick, black, dotted]
table {%
8 2.53373626047801
16 2.35505968672835
24 2.29467636405142
32 2.32248542146856
40 2.29201393933514
};
\addlegendentry{\textbf{\rsp[][\textbf]{} $\bm{\numrounds=8}$}}
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
8 2.55849078536099
16 2.3521355153069
24 2.30614395271632
32 2.34762555875491
40 2.28215573117707
};
\addlegendentry{\textbf{\rrsp[][\textbf]{} $\bm{\numrounds=4}$}}
\addplot [semithick, color0]
table {%
8 2.84523897323223
16 2.677880194081
24 2.59982363292901
32 2.62221254369764
40 2.54807234687754
};
\addlegendentry{random}
\addplot [semithick, color1]
table {%
8 2.68219640340884
16 2.59656980533227
24 2.57489075607254
32 2.65456079097416
40 2.63210529045662
};
\addlegendentry{myopic}
\addplot [semithick, color2]
table {%
8 2.54897944242204
16 2.33343086076026
24 2.29757642557278
32 2.3367321729912
40 2.2958723462484
};
\addlegendentry{sequential}
\end{axis}

\end{tikzpicture}


==> fig/target_tracking/normalized_solver_objectives.tex <==
% This file was created by tikzplotlib v0.8.7.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
height=\figureheight,
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={white!69.01960784313725!black},
xlabel={Objective (fraction of max)},
xmin=0.878939166426098, xmax=1.00576480159876,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ymin=0.5, ymax=7.5,
ytick style={color=black},
ytick={1,2,3,4,5,6,7},
yticklabel style={rotate=45,anchor=east},
yticklabels={random,myopic,
\textbf{\rsp[][\textbf]{} $\bm{\numrounds=2}$},
\textbf{\rsp[][\textbf]{} $\bm{\numrounds=4}$},
\textbf{\rsp[][\textbf]{} $\bm{\numrounds=8}$},
\textbf{\rrsp[][\textbf]{} $\bm{\numrounds=4}$},
sequential}
]
\addplot [black]
table {%
0.954787286286957 0.75
0.954787286286957 1.25
0.979055059400186 1.25
0.979055059400186 0.75
0.954787286286957 0.75
};
\addplot [black]
table {%
0.954787286286957 1
0.918680839191225 1
};
\addplot [black]
table {%
0.979055059400186 1
1 1
};
\addplot [black]
table {%
0.918680839191225 0.875
0.918680839191225 1.125
};
\addplot [black]
table {%
1 0.875
1 1.125
};
\addplot [black, mark=*, mark size=2, mark options={solid,fill opacity=0}, only marks]
table {%
0.918280288978132 1
0.918108995934431 1
0.91529252463204 1
0.890974614023062 1
0.912969454920479 1
0.916320355865791 1
0.890636006826516 1
0.906709209038523 1
0.915273640836571 1
0.884703968024856 1
0.904413518439951 1
0.909402495180871 1
0.912327675975411 1
0.909012620589598 1
0.917763084593916 1
0.910079068408362 1
0.908133155977623 1
0.916971106133061 1
0.91581185724962 1
0.918206123669863 1
0.90992095701077 1
0.894127994044857 1
0.91190662651904 1
0.892428996293456 1
0.916501431488103 1
0.916510658669993 1
0.917252434782623 1
};
\addplot [black]
table {%
0.965165629163503 1.75
0.965165629163503 2.25
0.989857796676087 2.25
0.989857796676087 1.75
0.965165629163503 1.75
};
\addplot [black]
table {%
0.965165629163503 2
0.928340231907027 2
};
\addplot [black]
table {%
0.989857796676087 2
1 2
};
\addplot [black]
table {%
0.928340231907027 1.875
0.928340231907027 2.125
};
\addplot [black]
table {%
1 1.875
1 2.125
};
\addplot [black, mark=*, mark size=2, mark options={solid,fill opacity=0}, only marks]
table {%
0.893429786100883 2
0.919638233237414 2
0.913503824204114 2
0.920749111720918 2
0.927699921512262 2
0.920881834906844 2
0.912112739981062 2
0.909271118577496 2
0.927812744207486 2
0.922146411825504 2
0.920698819235966 2
0.919977779902339 2
0.919289349916075 2
0.898340783179206 2
0.927551717636485 2
0.918322469353524 2
0.925802491300633 2
0.926343718077477 2
0.919437244020632 2
0.922806780259107 2
0.910174561011996 2
0.924458192644779 2
0.919512711117798 2
0.925449603657748 2
0.928002959225308 2
0.927503589261395 2
};
\addplot [black]
table {%
0.980248303792678 2.75
0.980248303792678 3.25
0.995752253704548 3.25
0.995752253704548 2.75
0.980248303792678 2.75
};
\addplot [black]
table {%
0.980248303792678 3
0.957050396478208 3
};
\addplot [black]
table {%
0.995752253704548 3
1 3
};
\addplot [black]
table {%
0.957050396478208 2.875
0.957050396478208 3.125
};
\addplot [black]
table {%
1 2.875
1 3.125
};
\addplot [black, mark=*, mark size=2, mark options={solid,fill opacity=0}, only marks]
table {%
0.953286822395311 3
0.945682932480194 3
0.956746583408294 3
0.946542851435617 3
0.951879853610367 3
0.954109042682895 3
0.953386755461595 3
0.953695680664574 3
0.955744953099545 3
0.951378058301163 3
0.954476271015511 3
0.95248994258515 3
0.953017825990497 3
0.937861736111546 3
0.954155406826504 3
0.9529908276563 3
0.940237759936091 3
0.946909794740719 3
0.950934627859721 3
};
\addplot [black]
table {%
0.981943678740974 3.75
0.981943678740974 4.25
0.997291526780195 4.25
0.997291526780195 3.75
0.981943678740974 3.75
};
\addplot [black]
table {%
0.981943678740974 4
0.959232427628575 4
};
\addplot [black]
table {%
0.997291526780195 4
1 4
};
\addplot [black]
table {%
0.959232427628575 3.875
0.959232427628575 4.125
};
\addplot [black]
table {%
1 3.875
1 4.125
};
\addplot [black, mark=*, mark size=2, mark options={solid,fill opacity=0}, only marks]
table {%
0.953321150917319 4
0.957003207618879 4
0.954985896136685 4
0.949939233472981 4
0.943823726014113 4
0.950189552724365 4
0.956177656850262 4
0.949979566489632 4
0.958181486927296 4
0.958310347435815 4
0.957559327357968 4
0.956610392930365 4
0.957063531383561 4
0.952814988615422 4
0.952634737753976 4
0.951334097453654 4
0.957440141043636 4
0.94209789584666 4
};
\addplot [black]
table {%
0.981928887909064 4.75
0.981928887909064 5.25
0.997484887488122 5.25
0.997484887488122 4.75
0.981928887909064 4.75
};
\addplot [black]
table {%
0.981928887909064 5
0.958610849657073 5
};
\addplot [black]
table {%
0.997484887488122 5
1 5
};
\addplot [black]
table {%
0.958610849657073 4.875
0.958610849657073 5.125
};
\addplot [black]
table {%
1 4.875
1 5.125
};
\addplot [black, mark=*, mark size=2, mark options={solid,fill opacity=0}, only marks]
table {%
0.954806118116995 5
0.95267106533295 5
0.953943714154223 5
0.949585034863671 5
0.947322139486869 5
0.941890497796306 5
0.94815758374126 5
0.952339181083388 5
0.952710450954984 5
0.949714515017142 5
0.939975637798977 5
0.955423484103426 5
0.954494096361914 5
0.946080938006907 5
0.943901666044695 5
0.949414375651824 5
0.954476598208151 5
0.957052998308692 5
0.952431394078387 5
0.958182176545859 5
0.942718548910982 5
0.954769229481822 5
};
\addplot [black]
table {%
0.981653037132224 5.75
0.981653037132224 6.25
0.997559681880982 6.25
0.997559681880982 5.75
0.981653037132224 5.75
};
\addplot [black]
table {%
0.981653037132224 6
0.957906902600171 6
};
\addplot [black]
table {%
0.997559681880982 6
1 6
};
\addplot [black]
table {%
0.957906902600171 5.875
0.957906902600171 6.125
};
\addplot [black]
table {%
1 5.875
1 6.125
};
\addplot [black, mark=*, mark size=2, mark options={solid,fill opacity=0}, only marks]
table {%
0.955806619653948 6
0.951215153276078 6
0.951754739792571 6
0.95473215597452 6
0.955310163365054 6
0.949406450272575 6
0.955574033697549 6
0.957338494356866 6
0.954552701303264 6
0.955028596084088 6
0.957057592274267 6
0.948264289017008 6
0.942818541865282 6
0.954669810744472 6
};
\addplot [black]
table {%
0.981593215305093 6.75
0.981593215305093 7.25
0.998463263398228 7.25
0.998463263398228 6.75
0.981593215305093 6.75
};
\addplot [black]
table {%
0.981593215305093 7
0.957007125404814 7
};
\addplot [black]
table {%
0.998463263398228 7
1 7
};
\addplot [black]
table {%
0.957007125404814 6.875
0.957007125404814 7.125
};
\addplot [black]
table {%
1 6.875
1 7.125
};
\addplot [black, mark=*, mark size=2, mark options={solid,fill opacity=0}, only marks]
table {%
0.95164684295425 7
0.953132083503165 7
0.94655618691 7
0.951041402533606 7
0.950621936571106 7
0.949416165492488 7
0.955839430594991 7
0.955238808562277 7
0.953376121194091 7
0.95191119242797 7
0.955353189680017 7
0.955280215907544 7
0.954083070155499 7
0.955207187430723 7
0.951006789289451 7
0.955902276689458 7
0.943251722259929 7
0.947917430557254 7
0.948435703628967 7
0.942473068539862 7
};
\addplot [color0]
table {%
0.968063591025807 0.75
0.968063591025807 1.25
};
\addplot [color0]
table {%
0.97826669395923 1.75
0.97826669395923 2.25
};
\addplot [color0]
table {%
0.98832324562467 2.75
0.98832324562467 3.25
};
\addplot [color0]
table {%
0.989810920883941 3.75
0.989810920883941 4.25
};
\addplot [color0]
table {%
0.990164835412537 4.75
0.990164835412537 5.25
};
\addplot [color0]
table {%
0.99046737965763 5.75
0.99046737965763 6.25
};
\addplot [color0]
table {%
0.990082800270504 6.75
0.990082800270504 7.25
};
\end{axis}

\end{tikzpicture}


==> fig/target_tracking/weights_by_number_of_robots.tex <==
% This file was created by tikzplotlib v0.8.7.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\pgfplotsset{set layers}
\begin{axis}[
height=\figureheight,
tick align=inside,
tick pos=left,
width=\figurewidth,
x grid style={white!69.01960784313725!black},
xmin=3.6, xmax=104.4,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Redundancy per robot},
ymin=8.98236207843095, ymax=49.865804015516,
ytick style={color=black}
]
\addplot [semithick, color0, mark=*, mark size=1, mark options={solid}]
table {%
8 10.8407003482985
16 24.5905367334807
24 36.0719841364776
32 41.7729690955876
40 36.1243044673496
48 48.0074657456485
56 46.0124414459563
64 35.8232283037079
72 32.8323116828888
80 33.1428971613599
88 35.7494800505622
96 26.7004014139884
};
\label{plot:one}
\addplot [semithick, color0, dashed, mark=*, mark size=1, mark options={solid}]
table {%
8 11.7387049109616
16 24.2905803860036
24 34.9773039071291
32 37.2397391126107
40 41.3929043035542
};
\label{plot:two}
\end{axis}

\begin{axis}[
axis y line*=right, % * removes arrow-head
height=\figureheight,
tick align=inside,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.97,0.03)}, anchor=south east, draw=white!80.0!black},
legend image post style={scale=0.5}, % resize legend entries
width=\figurewidth,
x grid style={white!69.01960784313725!black},
xlabel={Number of robots},
xmin=3.6, xmax=104.4,
xtick pos=left,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Objective value per robot},
ymin=2.43283255825653, ymax=3.20397863179633,
ytick={2.6, 2.8, 3.0},
ytick pos=right,
ytick style={color=black}
]
% Add prior legend entries
\addlegendimage{mark=*, semithick, color0, mark size=1, mark options={solid}}
\addlegendentry{redundancy, large-scale}
\addlegendimage{mark=*, semithick, dashed, color0, mark size=1, mark options={solid}}
\addlegendentry{redundancy, solver-trials}

\addplot [semithick, color1, mark=*, mark size=1, mark options={solid}]
table {%
8 2.46788465250834
16 2.80813227669389
24 2.95153878528677
32 3.0583830229871
40 3.02134852899013
48 3.14387493216099
56 3.1437930848549
64 3.10509514169753
72 3.09435593698503
80 3.11550793734448
88 3.16892653754452
96 3.1158062590958
};
\addlegendentry{objective, large-scale}
\addplot [semithick, color1, dashed, mark=*, mark size=1, mark options={solid}]
table {%
8 2.57998639421871
16 2.81653907973088
24 2.96341246005103
32 2.95430455825613
40 3.02001780419884
};
\addlegendentry{objective, solver-trials}
\end{axis}

\end{tikzpicture}

